Balancing Diversity and Risk in LLM Sampling: How to Select Your Method and Parameter for Open-Ended Text Generation

Sampling-based decoding strategies have been widely adopted for Large Language Models (LLMs) in numerous applications, targeting a balance between diversity and quality via temperature tuning and tail truncation. Considering the strong dependency of the candidate next tokens on different prefixes, recent studies propose to adaptively truncate the tail of LLMs' predicted distribution. Although improved results have been reported with these methods on open-ended text generation tasks, the results are highly dependent on the curated parameters and the limited exemplar text. In this paper, we propose a systematic way to estimate the capacity of a truncation sampling method by considering the trade-off between diversity and risk at each decoding step, based on our collected prefix tree which preserves the context of a full sentence. Our work offers a comprehensive comparison of existing truncation sampling methods and serves as a practical user guideline for their parameter selection.

==> Llama-2-7b-hf_means.tex <==
0.0,0.5013350196739742,7.810470695430424e-05,-7.329749689041512,-6.259918135832381,9.588522403366546e-05

==> evaluations/gpt2-xl_means0.tex <==
0.0,0.4809764715329639,0.0027633589006037015,-6.319868609079685,-5.168550424838,0.005182752060164212

==> evaluations/gpt2-xl_means1.tex <==
0.0,0.5007986500237257,0.007377779061106814,-4.886582645426277,-4.820198753570265,0.005012475005897973

==> tiksplot_test.tex <==
\begin{figure}
\centering
\vspace{3ex}
\begin{tikzpicture}[font=\tiny]
\begin{axis}[
        width=0.75\columnwidth,
        height=0.75\columnwidth,
        xlabel={Risk\phantom{$^{3}$}},
        ylabel={Recall},ylabel near ticks,
        xlabel near ticks,
        ymode=log, 
        %xmode=log,
        xmin=-0.2, xmax=10,
        ymin=-0.0001, ymax=1.1,
        mark size=0.1ex,
        legend entries={gpt2-xl-0, gpt2-xl-1},%
        legend style={draw=none,nodes={right}},
        legend pos=south east,
        clip marker paths=true
    ]
    % scatter plots
   %  \iffalse
    \addplot[
        only marks, mark=+, color=mycolor1!30
    ] table [
        col sep=comma,
        x index=0, y index=1
    ] {evaluations/gpt2-xl_risks_and_recalls_0_average_risk_05.txt}; 
         \addplot[
        only marks, mark=+, color=mycolor2!30
    ] table [
        col sep=comma,
        x index=0, y index=1
    ] {evaluations/gpt2-xl_risks_and_recalls_1_average_risk_05.txt};
    \addplot[
        only marks, mark=+, color=mycolor3!30
    ] table [
        col sep=comma,
        x index=0, y index=1
    ] {evaluations/gpt2-xl_risks_and_recalls_2_average_risk_05.txt};
%\fi
    % error bars
\end{axis}
\end{tikzpicture}
\caption{.}
\label{figure:test_comparison}
\end{figure}



    \iffalse

    \addplot[
        forget plot, only marks, color=mycolor1,
        error bars/.cd, x dir=plus, x explicit, y dir=plus, y explicit,
    ] table [
        col sep=comma,
        x index=0, y index=3,
        x error expr=\thisrowno{2}-\thisrowno{0}, y error expr=\thisrowno{5}-\thisrowno{3}
    ] {gpt2-xl_means.txt};
 \addplot[
        forget plot, only marks, color=mycolor1,
        error bars/.cd, x dir=minus, x explicit, y dir=minus, y explicit
    ] table [
        col sep=comma,
        x index=0, y index=3,
        x error expr=\thisrowno{0}-\thisrowno{1}, y error expr=\thisrowno{3}-\thisrowno{4}
    ] {gpt2-xl_means.txt};
    %\fi
    % median values
    \addplot[
        only marks, color=mycolor1
    ] table [
        col sep=comma,
        y index=1, x index=4,
    ] {evaluations/gpt2-xl_means0.txt};
    \fi
